Matrix Multiplicative Weights Updates in Quantum Zero-Sum Games: Conservation Laws & Recurrence

Recent advances in quantum computing and in particular, the introduction of quantum GANs, have led to increased interest in quantum zero-sum game theory, extending the scope of learning algorithms for classical games into the quantum realm. In this paper, we focus on learning in quantum zero-sum games under Matrix Multiplicative Weights Update (a generalization of the multiplicative weights update method) and its continuous analogue, Quantum Replicator Dynamics. When each player selects their state according to quantum replicator dynamics, we show that the system exhibits conservation laws in a quantum-information theoretic sense. Moreover, we show that the system exhibits Poincare recurrence, meaning that almost all orbits return arbitrarily close to their initial conditions infinitely often. Our analysis generalizes previous results in the case of classical games.

==> extensions.tex <==
In order to formalize a method for simulating and understanding quantum games, we propose a method to generate complex R matrices with the same eigenvalues as the values of the classical payoff matrix. This means that for any standard eigenbasis of a classical game, we create a new, complex eigenbasis where the eigenvalues are the same, but the eigenvectors are complex. Intuitively, this can be viewed as mapping a classical game matrix to the Hilbert space, effectively allowing generalizations of classically studied games to the semi-definite context. We introduce the following lemma, which describes a method to obtain a basis transformation to Hilbert space.

\begin{lemma}\label{lemma:hadamardtransform}
    For any $n\times n$ two player zero-sum game with classical payoff matrix $P$, let $\lambda_{i,j} = P_{i,j}$ and let $V$ and $W$ be unitary matrices of size $n\times n$.
    % $F_n$ be the $n\times n$ DFT matrix. 
    Then, the matrix $R$ defined as
    % $$R = \lambda^\top I (F_n \otimes F_n^*)$$
    \begin{equation}\label{eqn:basistransform}
        R = \sum_{i,j} \lambda_{i,j} (V_i\otimes W_j) (V_i^\dag \otimes W_j^\dag)
    \end{equation}
    produces a transformation from the classical payoff space $\mathcal{P}$ to the density matrix space $\mathcal{C}$. In particular, $R$
    is a complex $n^2\times n^2$ matrix which satisfies the following properties:
    \begin{itemize}
        \item The matrix $R$ is Hermitian.
        \item The eigenvalues of $R$ correspond to the elements of the classical payoff matrix $P$.
    \end{itemize}
\end{lemma}
\begin{proof}
    % \textcolor{}{}
    First note that equation \ref{eqn:basistransform} is equivalent to taking the following basis transformation:
    \[
    \sum_{i,j} \lambda_{i,j} (V_i\otimes W_j) (V_i^\dag \otimes W_j^\dag) = (V\otimes W){\Lambda} (V^\dag\otimes W^\dag)
    \]
    where $\Lambda = \begin{bmatrix}
    \lambda_{1,1} & \hdots & 0 \\
    \vdots & \ddots & \vdots\\
    0 & \hdots & \lambda_{n,n}
    \end{bmatrix}$ is the $n^2 \times n^2$ diagonal matrix formed by placing the elements of classical payoff matrix $P$ on the diagonal. Moreover, $V$ and $W$ are both unitary, so the tensor products $V\otimes W$ and $V^\dag\otimes W^\dag$ are also unitary. This holds because:
    \begin{align*}
        (V\otimes W)(V \otimes W)^\dag &= (V\otimes W)(V^\dag \otimes W^\dag)\\
        &= VV^\dag\otimes WW^\dag\\
        &= \mathbb{1}\otimes \mathbb{1} = \mathbb{1}
    \end{align*}
    
    This implies that $R$ can be written as a unitary diagonalization of the form $PDP^\dag$, where $P=(V\otimes W)$ and $D = \Lambda$. Hence $R$ is Hermitian and has real eigenvalues by the spectral theorem. In addition, by construction the eigenvalues of $R$ are the elements of the classical payoff matrix $P$. 
\end{proof}

Moreover, the initial conditions of a simulation of a two-player quantum zero-sum game can be similarly obtained by using the same orthonormal bases as in Lemma \ref{lemma:hadamardtransform} and applying a change of basis to the initial conditions in the standard basis. 
% Let $S_i$ be the n-vector of initial conditions for the $i$-th player. Then, the following transformation gives the new initial conditions $S'$:
% \begin{align}
%     S'_i &= \sum_{i} S_i (V_i V_i^*)
% \end{align}
% where $V_i$ are the orthonormal bases for each player. Note that this transformation guarantees that the new initial condition is a complex probability vector.

% Finally, we consider the properties of the transformed game. By Lemmas \ref{lemma:hermitianmwu} and \ref{lemma:hermitianrep}, given Hermitian initial conditions and R matrices, we can guarantee that the trajectories remain Hermitian.
% Our goal is to ultimately show that by selecting different $R$, we can guarantee that properties such as time average convergence to the Nash still hold for both MWU and replicator dynamics.

Using Lemma \ref{lemma:hadamardtransform} we can easily obtain quantum versions of classical games, and it follows from the basis transformation that MWU when applied using payoff observable $R$ results in trajectories that converge to the boundary in the transformed space. Likewise, the replicator trajectories exhibit recurrence in the transformed space.


==> intro.tex <==
% \cite{bondesan2021hintons}

% Modern literature about quantum game theory typically refers to the case where the mechanics of a classical game are changed (for example, allowing players to apply Hadamard gates to their pure states). This causes the pure strategies of the classical game to become an infinite set of pure strategies. However, our claim is that we can look at quantum games under a different paradigm. The idea of a mixed strategy has always been considered a probability distribution over the set of pure strategies in a fixed game. By looking at an expanded set of mixed strategies that include positive semidefinite Hermitian density matrices, we can gain a more intuitive understanding of the belief structure of game agents. Namely, each agent has a belief structure about the other agents' beliefs, in an inherently complex matrix space. However when a measurement is made (i.e. when the agent has to play a strategy), these matrices collapse into one result.


% The theory of learning in games has been studied extensively in the fields of theoretical computer science, economics and mathematics. 
% As an intersection of these fields, it provides a setting under which various emergent phenomena can be studied and better understood. 

The Nash equilibrium has always been a central concept in non-cooperative game theory. While the existence of Nash equilibria is well known in finite games where mixed strategies are allowed \cite{nash1951games}, it is less clear how to efficiently compute these equilibria themselves. Indeed, much work revolves around finding methods to solve for Nash equilibria in different contexts, as well as analyzing the complexity of solving for the Nash \cite{lemkehowson, daskalakis2009complexity}. 
% The study of learning in games is highly relevant 

% The study of learning in games is arguably as old a field as that of equilibrium computation \cite{fudenberg1998learning, borgers1997learning, friedman1991evolutionary, brown1951iterative}.
Despite the dominance of equilibrium computation in classical theory, recent works have begun to move towards attempting to understand the nature of learning in games \cite{fudenberg1998learning, borgers1997learning, friedman1991evolutionary, brown1951iterative}. 
% More specifically, the 
% provides evidence that the Nash equilibrium can be obtained as a result of learning and adaptation by one or more rational agents. This has ramifications in the fields of reinforcement learning \cite{Nowe2012MARL}, deep learning \cite{Schuurmans2016DeepLG} and control theory \cite{Marden2018Control}.
In particular, the dynamics of no-regret online learning algorithms have seen much interest in recent years. The family of regret-minimizing algorithms known as Follow The Regularized Leader (FTRL) have been studied extensively, both for discrete time \cite{bailey2018multiplicative, NEURIPS2018_90e13578, palaiopanos2017multiplicative} and continuous time \cite{mertikopouloscycles, flokas2019poincare, Piliouras2014OptimizationDC, perolat2020poincare} dynamics. 

Multiplicative Weights Update (MWU) is a ubiquitous update rule which has been studied under many guises \cite{littlestone1994weighted, freund1999adaptive, arora_multiplicative}.
% \citet{arora_multiplicative} studied the meta-algorithm known as Multiplicative Weights Update (MWU) in detail.
We focus on a generalization known as \emph{Matrix Multiplicative Weights Update} (MMWU), which changes the paradigm of standard MWU from cost vectors to cost matrices, and from probability vectors to density matrices. This generalization has been independently discovered and studied by \citet{tsuda2005matrix} as Matrix Exponentiated Gradient Updates and \citet{arora_multiplicative} as the Matrix Multiplicative Weights algorithm. 
% Moreover, several works study the idea of the \emph{Matrix Multiplicative Weights Update} (MMWU) algorithm, which changes the paradigm of standard MWU from cost vectors to cost matrices, and from probability vectors to density matrices. 
Applications of the MMWU algorithm include solving semi-definite programs (SDPs) \cite{arora2016combinatorial} and obtaining bounds on the sample complexity for learning problems in quantum computing \cite{kale2007efficient}. 
% Moreover, recent results such as \cite{jain2011qip} and \cite{du2019efficient} rely on MMWU.

% \citet{bailey2018multiplicative} showed that the oft-studied multiplicative weights algorithm (MWU) does not converge in day-to-day behaviour to the mixed Nash equilibrium when applied to two player zero-sum games. 

% Recent work has shown that leveraging semidefinite programs (SDPs) can allow for $\epsilon$-approximate Nash to be computed in polynomial time for two-player zero-sum games \cite{ahmadi2019semidefinite, laraki2009semidefinite, stein2007infinite}. In addition, the results have been shown to extend to a general class of semialgebraic games, providing a rich link between the worlds of optimization and game theory \cite{Parrilo2006PolynomialGA}. 

On the other side of the coin, quantum information theory has proved to be a useful tool in the fields of reinforcement learning and deep learning \cite{bondesan2021hintons, Daoyi_Dong_2008, dunjko2017advances}. This makes quantum game theory, the study of the exchange, measurement and processing of quantum information, a key part of the puzzle to better understand how quantum theory can change the landscape of computation. The basic results of classical game theory, such as von Neumann's minimax theorem and more have been shown to hold in the quantum context \cite{osti_1513429, Accardi_2020}, while recent work has shown analogous complexity and equilibrium results between classical and quantum games \cite{zhang2012quantum, bostanci2021quantum}. The closest paper to our own in the literature in the context of quantum games is \citet{jain2009parallel}, which analyzes the MMWU algorithm for quantum zero-sum games and proves time-average convergence to an approximate Nash equilibrium.
% Given the usefulness of MMWU in semidefinite programming, there is a natural confluence between the update rule and quantum computation. Specifically, quantum games can be perceived simply as classical games with an expanded mixed strategy space, which incorporates the cone of positive semidefinite matrices with trace $1$.

The theoretical advances surrounding quantum theory and online learning algorithms allow for very natural questions regarding the nature of learning in quantum games. Classical results have studied both the MWU algorithm and its continuous counterpart, \emph{replicator dynamics} from a learning perspective. 
% The family of regret-minimizing algorithms known as Follow The Regularized Leader (FTRL) have been studied extensively, both for discrete time \cite{bailey2018multiplicative, NEURIPS2018_90e13578, palaiopanos2017multiplicative} and continuous time \cite{mertikopouloscycles, flokas2019poincare, Piliouras2014OptimizationDC, perolat2020poincare} dynamics. 
\citet*{bailey2018multiplicative} showed that classical MWU does not converge in day-to-day behaviour to the mixed Nash equilibrium when applied to two player zero-sum games. \citet{mertikopouloscycles} showed that the orbits of players in zero-sum games exhibit Poincar\'{e} recurrence when using replicator dynamics. However, despite the plethora of discoveries in the classical world, much remains to be understood about online learning and more specifically the day-to-day dynamics of MMWU and its continuous counterpart in quantum games.
% For instance, while \citet{jain2009parallel} showed that MMWU converges in time average to an approximate Nash equilibrium, the limit behaviour of the dynamics in the quantum setting are not yet known.
% Furthermore, a quantum version of the MWU algorithm was presented in \cite{jain2009parallel}, which formulates the algorithm in the setting where each player sends a mixed quantum state to a referee, who then performs a measurement on the two states to determine payoffs. While time-average convergence to an approximate Nash is shown in their paper, the limit behaviour of the dynamics in the quantum setting are not yet known.

\paragraph{Contributions.} In this paper, we first study the dynamics of MMWU in quantum zero-sum games, utilizing tools from information theory and classical game theory. We provide bounds on the rate of change of the total quantum relative entropy in the system. This in turn motivates the introduction and study of quantum replicator dynamics. Drawing from multiple recent results in this direction, we show that the total quantum relative entropy in the system is a constant of motion. Furthermore, the dynamics exhibited by both players' trajectories do not converge to equilibrium (in the day-to-day sense) nor oscillate periodically, but rather exhibit a weaker form of periodicity known as \emph{Poincar\'e recurrence}. Our proof of this result departs from the standard classical method, representing our main technical novelty. Finally, we present several simulations which corroborate our theoretical results.

% Finally, we present several simulations which showcase our theoretical results, along with a method to convert classical game payoff matrices to the quantum setting.
% present a method to convert classical games which are often studied (such as Matching Pennies or Rock-Paper-Scissors) into semidefinite games/quantum games via basis transform, which aids in designing experiments and simulations.  

% \paragraph{Technical Novelty.}

\paragraph{Organization.} The rest of the paper is structured as follows: In Section \ref{sec:prelims}, we present fundamental concepts in both quantum and game theory. In addition, we introduce concepts in dynamical systems which will be helpful in our consequent analysis. Section \ref{sec:mwu} contains results pertaining to MMWU, while Section \ref{sec:replicator} contains the introduction to and analysis of quantum replicator dynamics. We present several experimental results in Section \ref{sec:experiments} and conclude with a discussion on future work in Section \ref{sec:conclusion}.




% - moving from classical probability distributions to quantum probability distributions.
% - Our key question: what does learning look like in this setting?
% - classical optimization problems can be solved with matrix multiplicative weights update
% - https://arxiv.org/pdf/0810.3150.pdf - formulation can be seen as a classical semidefinite program for zero sum game. It can also be seen as a quantum game.

% https://www.cs.princeton.edu/~arora/pubs/MWsurvey.pdf
% https://proceedings.neurips.cc/paper/2018/file/90e1357833654983612fb05e3ec9148c-Paper.pdf


